Performance Analysis of Matrix Multiplication for Deep Learning on the Edge

The devices designed for the Internet-of-Things encompass a large variety of distinct processor architectures, forming a highly heterogeneous zoo. In order to tackle this, we employ a simulator to estimate the performance of the matrix-matrix multiplication (GEMM) kernel on processors designed to operate at the edge. Our simulator adheres to the modern implementations of GEMM, advocated by GotoBLAS2, BLIS, OpenBLAS, etc., to carefully account for the amount of data transfers across the memory hierarchy of different algorithmic variants of the kernel. %Armed with this tool, A small collection of experiments provide the necessary data to calibrate the simulator and deliver highly accurate estimations of the execution time for a given processor architecture.

==> Figures/tmp <==
#FIG 3.2  Produced by xfig version 3.2.8b
Landscape
Center
Inches
Letter
100.00
Single
-2
1200 2
6 6375 150 11625 8775
6 9975 150 11625 1800
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10575 300 10575 1650
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 11025 300 11025 1650
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 10125 300 11475 300 11475 1650 10125 1650 10125 300
-6
6 6375 150 8025 1800
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6975 300 6975 1650
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 300 7425 1650
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 6525 300 7875 300 7875 1650 6525 1650 6525 300
-6
6 9975 1800 10725 3450
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 10125 1950 10575 1950 10575 3300 10125 3300 10125 1950
2 2 0 1 10 10 51 -1 20 0.000 0 0 -1 0 0 5
	 10125 1950 10575 1950 10575 2400 10125 2400 10125 1950
-6
6 8475 5100 10125 5850
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8625 5250 9975 5250 9975 5700 8625 5700 8625 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9075 5700 9075 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9525 5250 9525 5700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8775 5700 8775 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8925 5700 8925 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9225 5250 9225 5700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9375 5250 9375 5700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9675 5250 9675 5700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9825 5250 9825 5700
-6
6 10050 5175 11550 6675
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 11475 5250 11475 6600 10125 6600 10125 5250 11475 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 6150 11475 6150
2 2 0 1 11 11 51 -1 20 0.000 0 0 -1 0 0 5
	 11475 5250 11475 5400 10125 5400 10125 5250 11475 5250
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 5550 11475 5550
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 5700 11475 5700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 5850 11475 5850
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 6000 11475 6000
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 6300 11475 6300
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 6450 11475 6450
-6
6 7350 3525 7950 5025
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 7425 3600 7875 3600 7875 4950 7425 4950 7425 3600
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 3750 7875 3750
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 3900 7875 3900
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 4050 7875 4050
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 4800 7875 4800
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 4650 7875 4650
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 4500 7875 4500
2 2 0 1 19 19 51 -1 20 0.000 0 0 -1 0 0 5
	 7425 4200 7875 4200 7875 4350 7425 4350 7425 4200
-6
6 8550 3525 9150 5025
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8625 3600 9075 3600 9075 4950 8625 4950 8625 3600
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 3750 9075 3750
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 3900 9075 3900
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4050 9075 4050
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4500 9075 4500
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4650 9075 4650
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4800 9075 4800
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4350 9075 4350
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 4200 9075 4200
-6
6 8550 1875 10050 3375
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8625 1950 9975 1950 9975 3300 8625 3300 8625 1950
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9525 1950 9525 3300
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9075 1950 9075 3300
-6
6 8550 6825 8850 7425
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8625 6900 8775 6900 8775 7350 8625 7350 8625 6900
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 7050 8775 7050
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 8625 7200 8775 7200
2 2 0 2 0 13 50 -1 20 0.000 0 0 -1 0 0 5
	 8625 6900 8775 6900 8775 7050 8625 7050 8625 6900
-6
6 6450 6825 7950 7425
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 7875 6900 7875 7350 6525 7350 6525 6900 7875 6900
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6525 7050 7875 7050
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6525 7200 7875 7200
-6
6 6450 8475 7950 8775
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 6525 8550 7875 8550 7875 8700 6525 8700 6525 8550
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6675 8550 6675 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6825 8550 6825 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6975 8550 6975 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7125 8550 7125 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7275 8550 7275 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7425 8550 7425 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7575 8550 7575 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7725 8550 7725 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6600 8550 6600 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6750 8550 6750 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6900 8550 6900 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7050 8550 7050 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7200 8550 7200 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7350 8550 7350 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7500 8550 7500 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7650 8550 7650 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 7800 8550 7800 8700
-6
6 8850 8475 10350 8775
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8925 8550 10275 8550 10275 8700 8925 8700 8925 8550
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9075 8550 9075 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9225 8550 9225 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9375 8550 9375 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9525 8550 9525 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9675 8550 9675 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9825 8550 9825 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9975 8550 9975 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10125 8550 10125 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9000 8550 9000 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9150 8550 9150 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9300 8550 9300 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9450 8550 9450 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9600 8550 9600 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9750 8550 9750 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 9900 8550 9900 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10050 8550 10050 8700
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 10200 8550 10200 8700
-6
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 7425 1950 7875 1950 7875 3300 7425 3300 7425 1950
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 9225 3600 9675 3600 9675 4050 9225 4050 9225 3600
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 8625 300 9975 300 9975 1650 8625 1650 8625 300
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 7875 5250 7875 5700 6525 5700 6525 5250 7875 5250
2 2 0 2 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 10275 6900 10275 7050 8925 7050 8925 6900 10275 6900
2 1 0 1 0 7 50 -1 -1 0.000 0 0 -1 0 0 3
	 10125 2850 10575 2850 10575 2925
2 2 0 2 0 13 50 -1 20 0.000 0 0 -1 0 0 5
	 8625 8550 8775 8550 8775 8700 8625 8700 8625 8550
4 0 0 50 -1 0 14 0.0000 4 105 270 8175 2700 +=\001
4 0 0 50 -1 0 14 0.0000 4 105 270 8175 1050 +=\001
4 0 0 50 -1 0 14 0.0000 4 105 270 8175 5550 +=\001
4 0 0 50 -1 0 14 0.0000 4 105 270 8175 7200 +=\001
4 0 0 50 -1 0 14 0.0000 4 105 270 8175 8700 +=\001
4 0 0 50 -1 0 12 0.0000 4 105 240 8175 4200 +=\001
-6
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 450 Loop L1\001
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 2100 Loop L2\001
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 3750 Loop L3\001
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 5400 Loop L4\001
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 7050 Loop L5\001
4 0 0 50 -1 0 16 0.0000 4 255 930 -900 8700 Loop L6\001

